SARA: A Collection of Sensitivity-Aware Relevance Assessments

Large archival collections, such as email or government documents, must be manually reviewed to identify any sensitive information before the collection can be released publicly. Sensitivity classification has received a lot of attention in the literature. However, more recently, there has been increasing interest in developing sensitivity-aware search engines that can provide users with relevant search results, while ensuring that no sensitive documents are returned to the user. Sensitivity-aware search would mitigate the need for a manual sensitivity review prior to collections being made available publicly. To develop such systems, there is a need for test collections that contain relevance assessments for a set of information needs as well as ground-truth labels for a variety of sensitivity categories. The well-known Enron email collection contains a classification ground-truth that can be used to represent sensitive information, e.g., the Purely Personal and Personal but in Professional Context categories can be used to represent sensitive personal information. However, the existing Enron collection does not contain a set of information needs and relevance assessments. In this work, we present a collection of fifty information needs (topics) with crowdsourced query formulations (3 per topic) and relevance assessments (11,471 in total) for the Enron collection (mean number of relevant documents per topic = 11, variance = 34.7). The developed information needs, queries and relevance judgements are available on GitHub and will be available along with the existing Enron collection through the popular ir_datasets library. Our proposed collection results in the first freely available test collection for developing sensitivity-aware search systems.

==> content/abstract.tex <==
-

==> content/availability.tex <==
\begin{itemize}
  \item How to access the collection (ir-datasets?)
\end{itemize}

==> content/empirical_analysis.tex <==
\begin{itemize}
  \item Inter annotator agreement 
  \item Details / graphs of how many highly relevant, partially relevant, and not relevant emails there are 
\end{itemize}

==> content/introduction.tex <==
As identified by the UK government, valuable data which could be used to enable innovation and subsequently save public sector funds, currently cannot be made open and accessible as it potentially contains nationally critical, personal or commercially sensitive information \cite{government_release_collections}. Currently, in order to release such collections, every document must be manually reviewed by an expert reviewer and sensitive documents removed by hand \cite{mcdonald_active_learning}. This is due to the subtle and contextual nature of the sensitive information in unstructured free-text documents. In the era of born-digital documents where millions of documents are created daily, this process becomes infeasible due to time and financial constraints \cite{mcdonald_zero_tolerance}. Additionally, the notion of sensitivity changes over time. What is deemed sensitive at the time of the creation of a document might not be deemed to be sensitive in the future and vice-versa. \todo[inline]{This could be swapped for any example. Think this one is a bit long.}For example, information regarding the former president of Italy Silvio Berlusconi’s use of Panamanian offshore companies to hide assets from public scrutiny would be considered sensitive at the time. However, considering that this knowledge is in the public domain, it could be considered no longer sensitive. This is sensitive financial information, one of many categories and subcategories of information that could be considered sensitive. The United Kingdom Freedom of Information Act 2000 defines categories of sensitive information such as Legal Professional Privilege, Commercial Interests, and Personal Information. Within the Personal Information category, we can define sub-categories such as employment, health, and finance. See [TABLE] for a full list of sub-categories of Personal Information. 

It is therefore important that, to enable the development of sensitivity-aware search, we have a number of appropriate test collections which each provide documents containing a specific type of sensitive information to. There have been previous efforts to achieve this. For example, the TREC 2010 Legal Track provided a collection of documents that were labelled both for relevance and for legal privilege \cite{trec_legal_2010}. Legal privilege is a form of sensitive information, however as the documents were judged separately for both tasks there is not a large enough overlap to provide a useful collection for the development of sensitivity-aware search engines \cite{oard_collection}. \citet{oard_collection} created a collection annotated for both sensitivity and relevance. The Avocado Research Email Collection was used,  which contains a large number of emails from a defunct technology company and is held under a restricted research licence. This licence prevented the authors from using crowdsourcing and consequently, the authors made the judgments themselves based on two opposing personas that they devised. Additionally, access to the collection is not freely available. 

In this paper, we present the Enron Test Collection for Relevance and Sensitivity which is based on the Enron Email Collection. Enron was an energy company founded in 1985 which grew to dizzying heights, only to come crashing down in 2001 after a series of scandals and extensive fraudulent accounting. \todo[inline]{"Dizzying" and "crashing down" too informal?}As part of the investigation into the company by the Federal Energy Regulatory Commission after their bankruptcy, 600,000 emails made by employees were saved and subsequently publicly released. Over the years a number of emails have been removed by request from their author, but this remains the only freely available set of real emails which contain business and personal emails. A subset of the Enron email collection was labelled by students at UC Berkley - each email being reviewed by two people. Categories include logistic arrangements, employment arrangements and two categories for personal information. See [TABLE] for more details. We can assume that the categories “Purely personal” and “Personal but in a professional context” contain emails that are sensitive i.e. the author would not want them publicly available. Therefore, this collection adds another type of sensitivity to the existing test collections in the form of personal information sensitivities amongst business emails. 

==> content/pooling.tex <==
\begin{itemize}
  \item How which queries were chosen 
  \item Which search systems were used and implemented how
\end{itemize}

Gathering relevance judgments for every information need, email pair is financially infeasible. Therefore, pools of documents were created using 18 different retrieval models and the top documents in these pools were judged. The 18 retrieval models were made up of each combination of 3 different queries, 3 different retrieval models (DPH, BM25, and PL2) and using Bo1 query expansion or not. The queries were chosen from among those that were gathered from crowdsourcing. They were chosen to give the most diverse pool of documents to minimise the risk of relevant documents not being in the pool. A rank cutoff of 50 was used and the pools were deduplicated. 

==> content/related_work.tex <==
\begin{itemize}
    \item Sensitivity Classification
    \item Sensitivity aware search
    \item Pre-existing sensitivity aware search collections
\end{itemize}




==> content/relevance_and_sensitivity_judgments.tex <==
\begin{itemize}
  \item Explain how queries were collected through crowdsourcing
  \item Explain how relevance judgments were collected 
\end{itemize}

Two crowdsourcing tasks were carried out in order to generate this test collection. The first was to generate queries given an information need. Each crowdworker was shown 10 different information needs and asked to give a query that they would use to get information on that topic. Crowdworking was performed using the Prolific platform with filters that ensured workers were aged 18 or over and whose first language is English in order to ensure the quality of responses. Additionally, attention check questions were added to filter out workers that were not paying attention to the task. 

The second crowdsourcing task was to gather relevance judgments. This was carried out on the same platform with the same filters and attention checks. Workers were presented with 10 emails and asked to judge them as one of “Highly Relevant”, “Partially Relevant”, or “Not Relevant”, in relation to an information need that they were also presented. Workers were asked to enter the section of the email that influenced their decision. This was used as a further check that the workers were engaging in the task. 


==> content/sensitivity_classification.tex <==
\begin{itemize}
  \item Train a classifier on the collection and give details
  \item Shows that the collection is useful for sensitivity, good as it is a part of the problem of SAS
\end{itemize}

==> content/topic_creation.tex <==
\begin{itemize}
  \item Did LDA topic modelling 
  \item Also used those topics as 'bouncing off points' to search the emails and collect more topics
  \item Searched to ensure that I thought there was at least one relevant document per topic. One sensitive one too. 
\end{itemize}

Latent Dirichlet Allocation topic modelling was performed to generate topics on which information needs were based. This provided some clear topics that were used to generate information needs and also served as a jumping off point to guide the search in the emails. It was ensured that each topic had at least one related sensitive email in order to ensure that the collection is useful for developing sensitivity-aware ranking models. This process provided 100 topics each having at least one relevant sensitive document. Following on from this, information needs were written with the contents of the emails in mind. These information needs were provided to crowdworkers.
